Photophoretic Strength on Chondrules. 2. Experiment

Photophoretic motion can transport illuminated particles in protoplanetary disks. In a previous paper we focused on the modeling of steady state photophoretic forces based on the compositions derived from tomography and heat transfer. Here, we present microgravity experiments which deviate significantly from the steady state calculations of the first paper. The experiments on average show a significantly smaller force than predicted with a large variation in absolute photophoretic force and in the direction of motion with respect to the illumination. Time-dependent modeling of photophoretic forces for heat-up and rotation show that the variations in strength and direction observed can be well explained by the particle reorientation in the limited experiment time of a drop tower experiment. In protoplanetary disks, random rotation subsides due to gas friction on short timescales and the results of our earlier paper hold. Rotation has a significant influence in short duration laboratory studies. Observing particle motion and rotation under the influence of photophoresis can be considered as a basic laboratory analog experiment to Yarkovsky and YORP effects.

==> formel_kraft_aufheizen.tex <==
\begin{equation}
   %F(t) = a \, \mathrm{sech}\left(\frac{t-b}{c}\right)+d \left(1-e^{f-t/\tau}\right)+g
   F_z(t)=\begin{cases}
   a \, \mathrm{sech}\left(\frac{t-b}{c}\right) \left(1-e^{f-t/\tau}\right) + g & k\geq 0.4\,\mathrm{W/(m\, K)}\\
   \left(d-\frac{a}{e^{-t/b}+c}\right) \left(1-e^{f-t/\tau}\right) + g & \text{otherwise}
   \end{cases} \label{eq:F(t)}
\end{equation}
